ProPD: Dynamic Token Tree Pruning and Generation for LLM Parallel Decoding

Recent advancements in generative large language models (LLMs) have significantly boosted the performance in natural language processing tasks. However, their efficiency is hampered by the inherent limitations in autoregressive token generation. While parallel decoding with token tree verification, e.g., Medusa, has been proposed to improve decoding parallelism and efficiency, it often struggles with maintaining contextual relationships due to its independent token prediction approach and incurs significant verification overhead, especially with large tree sizes and batch processing. In this paper, we propose ProPD, an efficient LLM parallel decoding framework based on dynamic token tree pruning and generation. ProPD features an advanced early pruning mechanism to efficiently eliminate unpromising token sequences to improve verification efficiency. Additionally, it introduces a dynamic token tree generation algorithm to balance the computation and parallelism of the verification phase in real-time and maximize the overall efficiency across different batch sizes, sequence lengths, and tasks, etc. We verify ProPD across a diverse set of datasets, LLMs, and batch sizes and demonstrate ProPD consistently outperforms existing decoding algorithms by 1.1-3.2x.

==> docs/outline.tex <==
\section*{Outline}
\begin{itemize}
    \item Recent years have witnessed revolutional advancements in autoregressive large language models(LLMs), which can achieve start-of-the-art results in several generative natural language tasks, including summarization, machine translation and question answering. An autoregressive LLM is a neural network model that built upon transformer decoder blocks and consists of billions of parameters. The model is trained on a large corpus of texts to achieve the main goal of predicting the next word from the input text. Nevertheless, these LLMs have shown extreme low efficiency, for they have to generated one token per inference iteration. Each parameter must be loaded to generate a single token, making the transformer sampling process typically bound by memory bandwidth.

    \item To address the inefficiency in autoregressive token generation, a method called parallel decoding has been proposed. This approach tries to generate a list of potential tokens in some efficient ways. Then, the large language model only needs to confirm or reject this pre-generated sequence, which could potentially reduce inference latency.
    
    % In particular, speculative inference uses smaller autoregressive models to generate a list of tokens. Then the large model only needs to verify this speculative sequence of tokens.
    
    % \item However, it brings scheduling problems to hold multiple models in one system, and the proper small model is hard to determine. What's more, the small models are hard to be finetuned in the Reinforcement Learning from Human Feedback(RLHF) step, which is essential in LLM finetuning nowadays.

    \item %As a result, some researchers are exploring the use of the original model to predict several future tokens simultaneously. 
    Parallel decoding creates speculative sequences by anticipating multiple upcoming positions in the model’s output. Another strategy, the early-exiting structure, treats the initial layers of the model as a smaller model for generating speculative tokens. 

    \item Both methods possess distinct advantages and disadvantages. Parallel decoding can leverage the capabilities of large models to extract global information, for it generate the speculative tokens in the final layer. However, parallel decoding generates each predicted token independently, resulting in a lack of contextual relationships in the sequence.

    % \item  Early-exiting strategy is capable of generating tokens that conform to the contextually appropriate sequence for it predict in an autoregressive way, but it can only leverage the hidden states in the early layers and can only extract local information.

    \item The key to acceleration in parallel decoding lies in the length of accurately predicted sequence. Owing to the lower accuracy of speculative sequences of tokens, some methods produce multiple sequences for verification. Common prefixes are extracted and then the sequences can be combined as a token tree. Finally, all the sequences of a token tree can be verified simultaneously by making a single pass over the LLM's parameters. This mechanism can improve the average length of correct tokens predicted in each iteration. Due to the memory-bound feature of LLM inference, the token tree verification will not incur excessive overhead in a single batch. (\textcolor{blue}{insert a figure of token time against iteration time})
    
    \item However, in real-world serving systems, multi-batch inference is often required. When the batch size is large, the computational expense of tree decoding may become the primary bottleneck in latency. (\textcolor{blue}{insert a figure shows the latency when batch size is large and kv cache is long}). The memory consumption also increases when batch size is large and the KV cache is extensive. Continuing to verify large-scale token trees incurs significant computational overhead and occupies substantial memory. What's more, the accuracy of parallel decoding is also different under different tasks, making the trade-off between the benefits and overhead of parallel decoding more complex when changing the token tree size. \textcolor{blue}{(insert a figure of different acceptance length on different tasks)}
    
    \item To summarize, existing parallel decoding algorithm mainly has two problems:
    \begin{itemize}
        \item Parallel prediction of tokens at each position results in a loss of contextual relationships, thereby leading to an exponential growth in the size of the token tree.
        \item When the batch size and KV cache increase, the verification of token tree incurs a non-negligible computational overhead and memory consumption.
        \item Generate the token tree in a static way, regardless of runtime accuracy and overhead of parallel decoding. 
    \end{itemize}

    \item In order to address the contextual relationships of parallel decoding, we find an interesting phenomenon of autoregressive LLMs. \textcolor{blue}{(insert a score figure like song han)}As shown in xxx, the neighboring tokens tend to get larger attention scores in the early layers. Therefore, while the early layers of the model may not suffice for extracting global information to predict the correct tokens, they may be adequate for extracting local information to identify contextual relationships.

    \item Contributions
    \begin{itemize}
        \item Introduce early pruning mechanism into token tree verification to relieve the problem of loss of contextual relationships in parallel decoding.
        \item Propose dynamic token tree generation algorithm based on runtime batch size, KV cache length and parallel decoding accuracy.
        \item Compared to previous methods, achieve better acceleration even when the barch size is large.
    \end{itemize}

    \item Methods \textcolor{blue}{(insert an overview figure)}
    \begin{itemize} 
        \item formal illustration of parallel tree decoding
        \item early pruning of token tree \textcolor{blue}{(insert an illustration figure of early pruning structure)}
        \item dynamic token tree generation \textcolor{blue}{insert an algorithm to illustrate the whole workflow}
    \end{itemize}

    \item Experiments
    \begin{itemize}
        \item 3 datasets, 2 model size(7b \& 33b)
        \item baseline \& medusa
        \item speedup comparison(dataset, model size, batch size)
        \item Ablation study
        \begin{itemize}
            \item prune accuracy (the acceptance length keeps)
            \item w/o prune and w/o dynamic generation
        \end{itemize}
    \end{itemize}
    
\end{itemize}


==> docs/proposal.tex <==
Block decoding vs speculative decoding vs early exiting
\begin{itemize}
    \item Block decoding predicts the next $d$ output tokens, i.e., $\{y_{t+1}, \ldots, y_{t+d}\}$, based on $\{y_0, \ldots, y_{t-1}, y_t\}$.
    \item Speculative decoding leverages a small model to generate the drafts for the next $d$ tokens and then, uses the large model to verify the tokens.
    \item Early exiting predicts the next token through the output hidden states of early layers. 
\end{itemize}

Problems with block decoding:
\begin{itemize}
    \item The generation of $y_{t+i}$ for $i \geq 2$ cannot consider the previous tokens within the block, i.e., $\{y_{t+1}, \ldots, y_{t+i-1}\}$. This limits the acceptance rate for block decoding.
    \item To generate and verify top $k$ predictions for each token, the total number of sequences increases exponentially with both $k$ and the block size $d$, which drastically increases the latency for verification.
    \item Any other problems with block decoding?
\end{itemize}

Problems with and potential of early exiting:
\begin{itemize}
    \item Cannot utilize the previous final hidden states
    \item auto-regressive
    \item Uncapable of predicting the correct next token, but capable of pruning the wrong sequences.
\end{itemize}

Improving block decoding with partial auto-regressive block decoding?
\begin{itemize}
    \item To better predict and increase the acceptance rate of $y_{t+i}$ for $i \geq 2$, we hope to incorporate $\{y_{t+1}, \ldots, y_{t+i-1}\}$ into the block decoding process.
    \item To incorporate previous tokens and enable auto-regressive decoding, at least one transformer layer is needed. Then, we need to determine 1) whether one separate transformer layer is needed for these tokens (or what are the parameters that can be shared); 2) whether the final projection layer can be shared; 3) any space for scheduling optimization.
    \item Meanwhile, we also need to determine how to verify and generate tokens simultaneously and how to deal with incorrect predictions, e.g., directly skip (including both greedy sampling and batch sampling) or iterative refinement.
\end{itemize}
